Spectral analysis for nonstationary audio

A new approach for the analysis of nonstationary signals is proposed, with a focus on audio applications. Following earlier contributions, nonstationarity is modeled via stationarity-breaking operators acting on Gaussian stationary random signals. The focus is on time warping and amplitude modulation, and an approximate maximum-likelihood approach based on suitable approximations in the wavelet transform domain is developed. This paper provides theoretical analysis of the approximations, and introduces JEFAS, a corresponding estimation algorithm. The latter is tested and validated on synthetic as well as real audio signal.

==> preamble.tex <==
\usepackage[utf8]{inputenc} % accents 8 bits dans le fichier
%\usepackage[T1]{fontenc}
\usepackage{stfloats}
%\usepackage[english,french]{babelfr}   
\usepackage{mathrsfs}  

%\usepackage{url}
\usepackage{graphicx}
\usepackage{subfig}
\usepackage{picture}
\usepackage[usenames]{color}
\usepackage{amsfonts,amsmath, amssymb}
\usepackage{algorithm,algorithmic}
\usepackage{soul}
\usepackage[english]{babel}
%\usepackage{hyperref}
\usepackage{enumitem}

\usepackage{pdftricks}
\begin{psinputs}
   \usepackage{pstricks,pst-plot,pstricks-add}
   \usepackage{multido}
\end{psinputs}

\usepackage{textcomp}

%\usepackage[style=ieee]{biblatex}
%\AtEveryBibitem{%
%  \clearfield{issn} % Remove issn
%  \clearfield{doi} % Remove doi
%
%  \ifentrytype{online}{}{% Remove url except for @online
%    \clearfield{url}
%  }
%}

\usepackage{epstopdf}

\newtheorem{theorem}{Theorem}
\newtheorem{remark}{Remark}

%\newcommand{\mytilde}{\raise.17ex\hbox{$\scriptstyle\mathtt{‌​\sim}$}}
\setlength{\itemindent}{-1.5in}
